Free-Riding the Agentic Web: A Systematic Security Analysis of x402 Payments

The x402 protocol has crossed from prototype to infrastructure for the agentic web, driving 130 million all-time transactions and embedded in Google Cloud, Cloudflare, and Stripe. Yet bridging synchronous HTTP requests with asynchronous blockchain finality creates state-synchronization challenges, and x402's security has so far been examined only in piecemeal vendor disclosures. It is moreover not one artefact but a stack of an HTTP semantic, per-chain schemes, and a long tail of SDK and deployment choices whose required guarantees prior work has not established. We perform a systematic security analysis organized around five invariants grounded in specifications, literature, and vendor expectations, resolving every violation to the responsible layer. We identify four flaw classes: cross-resource substitution, duplicate-settlement race (independently corroborated by subsequent third-party reports), allowance overdraft, and denial of settlement. Against official SDKs and a production deployment, these reach resource-leakage ratios up to 100%. For pay-per-token scheme we prove a structural limit: no output-only pricing can be both fair to honest users and bounded against inflation of the hidden "thinking" tokens, the price of fairness being a $\sqrt{1+\Theta}$ manipulation gap. We propose per-flaw mitigations and a defense triple with provable guarantees, cutting per-call reasoning cost by 47% and inverting attacker leverage from 8.7$\times$ to 0.9$\times$ at only 2.8% overhead. All findings have been disclosed.

==> fig/tokenization-correction.tex <==
\begin{table}[t]
\caption{Tokenization correction factors: naive chars/4 vs.\ BPE tokenizer. Per-model (left) and per-category (right) mean error and correction factor.}
\label{tab:tokenization}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{minipage}[t]{0.49\columnwidth}\centering
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{By Model} & \textbf{Err} & \textbf{Factor} \\
\midrule
Gem-flash & +1.2\% & 0.988 \\
Gem-pro   & +42.4\% & 0.702 \\
GPT-5.2   & +3.2\% & 0.969 \\
GPT-5.3   & $-$4.6\% & 1.048 \\
Opus-4.6  & $-$3.7\% & 1.039 \\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{0.49\columnwidth}\centering
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{By Category} & \textbf{Err} & \textbf{Factor} \\
\midrule
Adver.   & +29.0\% & 0.775 \\
Code     & +15.6\% & 0.865 \\
Creative & +7.9\% & 0.927 \\
Factual  & $-$26.6\% & 1.363 \\
Meta     & +12.5\% & 0.889 \\
Reason   & $-$5.4\% & 1.057 \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}


==> fig/transferability.tex <==
\begin{table}[t]
\caption{Cross-model attack transferability: 5 adversarial prompts $\times$ 3 models. All prompts achieve \textbf{138--466$\times$ inflation} on at least 2 models; ``ref.'' = model refused.}
\label{tab:transferability}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrc@{}}
\toprule
\textbf{Prompt} & \textbf{GPT-5.2} & \textbf{Gem.\ Pro} & \textbf{Gem.\ Flash} & \textbf{Mean} & \textbf{Class} \\
\midrule
adv-01 & 229$\times$ & \textbf{414$\times$} & 138$\times$ & 260$\times$ & universal \\
adv-02 & 146$\times$ & \textbf{466$\times$} & 149$\times$ & 254$\times$ & universal \\
adv-03 & 242$\times$ & \textbf{397$\times$} & ref. & 320$\times$ & universal \\
adv-04 & 302$\times$ & \textbf{448$\times$} & ref. & 375$\times$ & universal \\
adv-05 & \textbf{194$\times$} & ref. & 144$\times$ & 169$\times$ & universal \\
\bottomrule
\multicolumn{6}{@{}p{8.3cm}@{}}{\scriptsize Gem.\ models saturate near output cap (${\sim}$10K chars); variation from tokenization differences.}
\end{tabular}
\end{table}

